Distributed Linear Programming on GPU Clusters at Extreme Scale

Large linear programs can exceed the memory of a single compute node. Although first-order methods replace sparse factorizations with GPU-suited matrix-vector products, other solver phases can reintroduce a single-node memory limit. We present SHARDLP, a distributed GPU LP solver that keeps the matrix and primal-dual state partitioned from sharded input through solution output. On the Google PDLP benchmark, SHARDLP solves ten of eleven instances, compared with eight in the published CPU PDLP study. On the largest benchmark, eight H200 GPUs solve a 1.185-billion-variable, 6.338-billion-nonzero LP in 9.9 minutes; the published CPU experiment reports 21.06 hours on different hardware. Beyond this benchmark, separately checked multi-node solves reach up to 13.604 billion variables and 40.807 billion nonzeros, while validated executions span up to 76 GPUs across 29 compute nodes. For column-partitioned solves, support-aware communication skips GPUs that store no coefficients for a row; on an LP with 2.76 billion nonzeros, it cuts modelled communication by 92.97% and improves solver time by 1.27x-1.52x. The code for SHARDLP is available at https://github.com/ArnaudDeza/ShardLP.

==> figures/figure1_candidate.tex <==
\begingroup
\definecolor{FigureBlue}{RGB}{0,114,178}
\definecolor{FigureOrange}{RGB}{213,94,0}
\definecolor{FigureTeal}{RGB}{0,133,119}
\definecolor{FigureRose}{RGB}{180,76,96}
\begin{tikzpicture}[
  x=1cm,y=1cm,
  font=\scriptsize,
  rootbox/.style={draw=black!34,fill=black!1,rounded corners=1.6pt,
                  minimum width=2.80cm,minimum height=1.12cm,
                  inner sep=2pt,align=center},
  workerbox/.style={draw=black!30,fill=white,rounded corners=1.6pt,
                    minimum width=2.80cm,minimum height=.84cm,
                    inner sep=1.5pt,align=center},
  chip/.style={draw=black!38,fill=FigureBlue!8,rounded corners=.7pt,
               minimum width=.40cm,minimum height=.34cm,inner sep=0pt},
  nodebox/.style={draw=black!32,fill=black!1,rounded corners=1.4pt,
                  line width=.48pt},
  matrixblock/.style={draw=black!40,fill=white,rounded corners=.7pt,
                      minimum width=1.16cm,minimum height=.58cm,
                      inner sep=1pt,align=center},
  xblock/.style={draw=FigureBlue!70,fill=FigureBlue!8,
                 rounded corners=.8pt,minimum width=1.16cm,
                 minimum height=.34cm,inner sep=.8pt,
                 text=FigureBlue!80!black,align=center},
  axblock/.style={draw=FigureBlue!70,fill=FigureBlue!8,
                  rounded corners=.8pt,minimum width=.92cm,
                  minimum height=.34cm,inner sep=.8pt,
                  text=FigureBlue!80!black,align=center},
  gradblock/.style={draw=FigureOrange!78!black,fill=FigureOrange!8,
                    rounded corners=.8pt,minimum width=1.16cm,
                    minimum height=.34cm,inner sep=.8pt,
                    text=FigureOrange!72!black,align=center},
  axflow/.style={-{Latex[length=1.6mm,width=1.0mm]},
                 draw=FigureBlue!80,line width=.62pt},
  rowtap/.style={draw=FigureBlue!80,line width=.62pt},
  gradflow/.style={-{Latex[length=1.6mm,width=1.0mm]},
                   draw=FigureOrange!84!black,line width=.62pt,dashed},
  lifeline/.style={-{Latex[length=1.6mm,width=1.0mm]},
                   draw=FigureTeal!76!black,line width=.60pt}
]

\path[use as bounding box] (0,0) rectangle (14.00,5.10);

% One divider, no dashboard-style outer cards.
\draw[draw=black!24,line width=.42pt] (3.45,.18) -- (3.45,4.92);

% --------------------------------------------------------------------------
% (a) A distributed iteration surrounded by a rooted lifecycle.
% --------------------------------------------------------------------------
\node[anchor=west,font=\small\bfseries] at (.22,4.78)
  {(a) Rooted lifecycle};

\node[rootbox] (root) at (1.70,3.55)
  {\textbf{one compute node}\\[-1pt]
   full $A,x,y$\\[-1pt]
   input $\boldsymbol{\cdot}$ scale $\boldsymbol{\cdot}$ recover};

\node[workerbox] (workers) at (1.70,1.92) {};
\node[font=\scriptsize\bfseries,text=black!74] at (1.70,2.17)
  {PDHG on GPUs};
\foreach \xc/\id in {.78/0,1.39/1,2.01/2,2.62/3}
  \node[chip] at (\xc,1.78) {\id};

% Separate one-way arrows keep the lifecycle labels off the communication path.
\draw[-{Latex[length=1.65mm,width=1.05mm]},draw=black!56,line width=.58pt]
  (1.48,2.93) -- (1.48,2.40);
\draw[-{Latex[length=1.65mm,width=1.05mm]},draw=black!56,line width=.58pt]
  (1.84,2.40) -- (1.84,2.93);
\node[anchor=west,text=black!74] at (2.03,2.77) {scatter};
\node[anchor=west,text=black!74] at (2.03,2.55) {gather};

\draw[draw=FigureRose!72!black,fill=FigureRose!7,rounded corners=1.4pt,
      line width=.48pt] (.17,.27) rectangle (3.23,.91);
\node[align=center,font=\scriptsize,
      text=FigureRose!80!black] at (1.70,.59)
  {{\fontsize{6.5}{7.0}\selectfont per-node memory ceiling}\\[-1pt]
   $O(\operatorname{nnz}(A)+m+n)$};
\draw[-{Latex[length=1.55mm,width=1.0mm]},draw=FigureRose!78!black,
      line width=.55pt]
  (root.west) -- (.09,3.55) -- (.09,1.05) -- (.35,1.05) -- (.35,.91);

% --------------------------------------------------------------------------
% (b) Persistent two-dimensional ownership.
% --------------------------------------------------------------------------
\node[anchor=west,font=\small\bfseries] at (3.76,4.78)
  {(b) Persistent ownership};
\node[anchor=west,font=\scriptsize,text=black!74]
  at (3.79,4.43) {3 compute nodes $\times$ 2 GPUs/node; one MPI rank per GPU};

% Each band is one physical compute node in the allocation.
\draw[nodebox] (4.40,1.00) rectangle (6.10,4.22);
\draw[nodebox] (6.35,1.00) rectangle (8.05,4.22);
\draw[nodebox] (8.30,1.00) rectangle (10.00,4.22);
\node[font=\scriptsize,text=black!74] at (5.25,4.04) {node 0};
\node[font=\scriptsize,text=black!74] at (7.20,4.04) {node 1};
\node[font=\scriptsize,text=black!74] at (9.15,4.04) {node 2};

% Each compute node contains two GPU-resident MPI ranks, one per process-grid row.
\foreach \cc/\xc in {0/5.25,1/7.20,2/9.15} {
  \node[xblock] (x\cc) at (\xc,3.64) {$x_{J_{\cc}}$};
  \node[matrixblock] (a0\cc) at (\xc,2.91) {$A_{0\cc}$};
  \node[matrixblock] (a1\cc) at (\xc,2.12) {$A_{1\cc}$};
  \node[gradblock] (g\cc) at (\xc,1.23) {$(A^{\mathsf T}y)_{J_{\cc}}$};
  \draw[gradflow] (a0\cc.south) -- (a1\cc.north);
  \draw[gradflow] (a1\cc.south) -- (g\cc.north);
}
\node[anchor=east,text=FigureOrange!78!black] at (4.14,2.91)
  {$y_{I_0}$};
\node[anchor=east,text=FigureOrange!78!black] at (4.14,2.12)
  {$y_{I_1}$};

% Blue buses make every contribution to each grid-row reduction explicit.
\node[axblock] (ax0) at (10.82,2.91) {$(Ax)_{I_0}$};
\node[axblock] (ax1) at (10.82,2.12) {$(Ax)_{I_1}$};
\foreach \cc/\xt in {0/5.98,1/7.93,2/9.88} {
  \draw[rowtap] (a0\cc.east) -- (\xt,2.91) -- (\xt,3.31);
  \draw[rowtap] (a1\cc.east) -- (\xt,2.12) -- (\xt,1.62);
}
% White under-strokes prevent solid-blue and dashed-orange crossings from
% looking like additional summation junctions.
\draw[draw=white,line width=1.55pt]
  (5.98,3.31) -- (10.18,3.31) -- (10.18,2.91) -- (ax0.west);
\draw[axflow]
  (5.98,3.31) -- (10.18,3.31) -- (10.18,2.91) -- (ax0.west);
\draw[draw=white,line width=1.55pt]
  (5.98,1.62) -- (10.18,1.62) -- (10.18,2.12) -- (ax1.west);
\draw[axflow]
  (5.98,1.62) -- (10.18,1.62) -- (10.18,2.12) -- (ax1.west);
\node[anchor=west,align=left,text=FigureBlue!82!black,
      font=\scriptsize\bfseries] at (11.42,2.52)
  {row reductions\\[-1pt]assemble $Ax$};
\node[anchor=west,align=left,text=FigureOrange!80!black,
      font=\scriptsize\bfseries] at (10.22,1.23)
  {column reductions\\[-1pt]assemble $A^{\mathsf T}y$};

% The lifecycle is one unobtrusive rail, not a third panel.
\draw[lifeline] (3.95,.48) -- (13.55,.48);
\foreach \xc/\lab in {4.20/input,5.98/scale,7.76/PDHG,9.54/polish,
                      11.32/recover,13.10/output} {
  \draw[draw=FigureTeal!76!black,fill=white,line width=.52pt]
    (\xc,.48) circle (.075);
  \node[font=\scriptsize,text=black!72] at (\xc,.73) {\lab};
}
\node[font=\scriptsize\bfseries,text=FigureTeal!72!black] at (8.65,.20)
  {same ownership throughout};

\end{tikzpicture}
\endgroup

